Deep Polycuboid Fitting for Compact 3D Representation of Indoor Scenes

This paper presents a novel framework for compactly representing a 3D indoor scene using a set of polycuboids through a deep learning-based fitting method. Indoor scenes mainly consist of man-made objects, such as furniture, which often exhibit rectilinear geometry. This property allows indoor scenes to be represented using combinations of polycuboids, providing a compact representation that benefits downstream applications like furniture rearrangement. Our framework takes a noisy point cloud as input and first detects six types of cuboid faces using a transformer network. Then, a graph neural network is used to validate the spatial relationships of the detected faces to form potential polycuboids. Finally, each polycuboid instance is reconstructed by forming a set of boxes based on the aggregated face labels. To train our networks, we introduce a synthetic dataset encompassing a diverse range of cuboid and polycuboid shapes that reflect the characteristics of indoor scenes. Our framework generalizes well to real-world indoor scene datasets, including Replica, ScanNet, and scenes captured with an iPhone. The versatility of our method is demonstrated through practical applications, such as virtual room tours and scene editing.

==> sec/7_applications.tex <==
\section{Applications} 
To showcase the potential of our method in practical applications, we present two key applications based on our reconstructed polycuboids: \textbf{room tour and room editing}.

\textbf{Room Tour:} We execute a room tour with various viewpoints, as depicted in Fig. \ref{fig:app_roomtour}. Despite the simplified geometry, our texture-mapped rooms provide clean and visually appealing renderings that closely resemble the original scanned data, offering a seamless virtual exploration experience.

\textbf{Room Editing:} We further demonstrate the capabilities of our method through a range of room editing scenarios, showcased in Fig. \ref{fig:app_editing}. 
In the first row, we can delete existing table reconstructed using polycuboid, and put a new table.
In the second row, we highlight the ability to reposition objects within the scene. We remove existing objects and relocate the reconstructed sofa that was on the other side.
Given the potential to manipulate and adjust virtual environments with such ease, our approach holds great promise for a range of industries, including interior design, and AR/VR applications.
 
